Analytics and Machine Learning in Vehicle Routing Research

The Vehicle Routing Problem (VRP) is one of the most intensively studied combinatorial optimisation problems for which numerous models and algorithms have been proposed. To tackle the complexities, uncertainties and dynamics involved in real-world VRP applications, Machine Learning (ML) methods have been used in combination with analytical approaches to enhance problem formulations and algorithmic performance across different problem solving scenarios. However, the relevant papers are scattered in several traditional research fields with very different, sometimes confusing, terminologies. This paper presents a first, comprehensive review of hybrid methods that combine analytical techniques with ML tools in addressing VRP problems. Specifically, we review the emerging research streams on ML-assisted VRP modelling and ML-assisted VRP optimisation. We conclude that ML can be beneficial in enhancing VRP modelling, and improving the performance of algorithms for both online and offline VRP optimisations. Finally, challenges and future opportunities of VRP research are discussed.

==> _chance.tex <==

Chance-constrained programs are different from the stochastic programming and robust optimization.  It assumes that constraints are satisfied to some degree, measured by probabilities, rather than fully met. In VRPs, the chance-constrained CVRPs consider vehicle routes that satisfy the customer demands along each route with a pre-specified probability. This problem is typically solved using branch-and-cut methods. 

%Chance constrained VRP involves the stochastic variables in VRP modeling such as VRP with stochastic demand. 
\cite{dinh2018exact} model the stochastic demand of customers as a joint normal distribution or a given discrete distribution. 
In particular, such modelling allows correlation between customer demands rather than independent demands. A branch-and-cut-and-price (BCP) algorithm is used to tackle the problem. A routes relaxation technique is proposed in order to price through dynamic programming. The experiments demonstrated this approach's ability to solve the distributionally robust chance constrained vehicle routing problems (CCVRPs). 

\cite{ghosal2020distributionally} focus on the distributionlly robust chance-constrained CVRP, which considers the probability distribution of the customer demand is partially known. The customer demands are modeled as the distribution based on ambiguity sets. Several first-order and second-order moment ambiguity sets are investigated and branch-and-cut schemes can be used to solve it. The experiments demonstrated the good scalability of distributionlly robust CVRP. 

\cite{li2010vehicle} studied a version of VRP where the service and travel times are stochastic and time window constrains are involved. Such problem is then formulated as a chance constrained programming model and a stochastic programming model with recourse. The author assigned confidence level for both time window and driving duration of each route. The tabu search algorithm is used to solve the problem. 

Simlarly, \cite{gutierrez2018multi} also focus on VRP with stochastic service and travel times and time windows. In this work, the arrival times are estimated by a log-normal approximation. A multi-population memetic algorithm (MPMA) is then proposed and solve the problem.  

\cite{wu2020chance} studied VRP for application of wet waste collections. In this work, chance constrained programming is used to model the uncertainty of waste generation rate and make it deterministic. A hybrid algorithm consisted of particle swarm optimization (PSO) and simulated annealing (SA) are used for the optimization.

\cite{men2019chance} focused on the HazMat capacitated vehicle routing problem (H-CVRP). This problem aims at minimizing the risk of transportation. The author used chance constrained programming to transfer the uncertainty of risk parameters into a deterministic form. A simulated annealing algorithm is designed to optimize the objective function. 


==> _constructive.tex <==
\section{Constructive}

Generating valid tour constructively is considered as a natural way of solving VRP problems. (non-ML historical review) The VRP problem is considered as a process of sequentially select nodes with some specified policy. The prosperity of machine learning inspires researchers to use parameterized, learning-based policy to select nodes. 

Vinyals et.al. started to apply machine learning methods to solve typical combinatorial optimization problems. They purpose Pointer Network as a tool to solve sequential decision problem, including VRP and its variant\cite{vinyals2015pointer}. The pointer network uses encoder-decoder structure based on recurrent neural network(RNN). In last step, instead of calculating probability distribution over dictionary, they calculate the distribution over the set containing all available nodes to satisfy the constraints. Although tested only on a small set of problems, the proposed method proved that a purely neural-network based learning solution can solve combinatorial optimization problems by constructing the solution.



==> _forecast.tex <==

% model param setting
In this subsection, we will discuss a more loose connection between machine learning 
and VRP problem. Research works in this area are not likely to use machine learning 
methodology to solve related problem, but as a tool to reflect and analysis data that 
related to problem solution. A rough classification by \cite{talbi2016combining} divide
such combination into low-level, which is highly related to hyperparameter tuning; and 
high-level, where machine learning is applied to help modeling and provide certian
context for metaheuristics. In this section, we will mainly focuse on machine learning assisted predictive model for uncertainties in VRP, and machine learning based model fine-tuning methods.

%----------------------------
\subsubsection{Predictive Model for Uncertainties in VRP}

So far, a great number of methods have proposed to solved classic VRP and most of them are demonstrated by generating high-quality solutions. However, most of these methods fail to work in realistic scenarios because of the over-simplification of the real-world constrains and logistics. For example, the elements such as customer demands, customer appearance, and travel time may not be deterministic. Therefore, more sophisticated approaches are required to model and solve these problems. 

\cite{ce2010solving} made a basic classification by analysing customer's demands and introduced corresponding data mining techniques for each cases. 
\cite{markovic2005using} used neural network to predict customers' stochastic demand based on historical data, while \cite{snoeck_route_2020} applied probabilistic graphical model to predict constrained customers for routing problems. \cite{musolino2013travel} developed a simulation-based method to forecast the travel time for an emergency vehicles routing problem. 
\cite{li2018data} applied a data-driven search algorithm to improve traditional 
metaheuristics methods for large-scale manufacturing logistic problems in real-world 
industry practice. In the VRP part, 
they learned a multinomial transition matrix by updating from historical expert data and 
generate valid solution by sampling from the matrix. 

 \cite{calvet2016combining} considered a  realistic VRP setting where customers have different demands to different assigned depots. The matching between heterogeneous depots and customers with stochastic demand could significantly affect the profit of the company. Thus, several regression models which estimate the customer demands based on their assigned depot are used to support the market segmentation strategy. 
 
 In dynamic VRP, customer's availability indicates the available service time window of each customer, which is one of the important aspects that cause the dynamism in dynamic VRP. \cite{kucharska2019dynamic} focused on this dynamism and used algebraic-logical meta-model (ALMM) to solve dynamic VRP with predicted customer availability. 

Another common used modelling approach addressing uncertainties in VRP is  rolling horizon planning. In such framework, problem is solved iterativelly over a planning horizon that shifts forward a fix or unfixed time span at each step. At each iteration, some of the uncertainties of the problem are estimated with historical data. \cite{cordeau2015rolling} used this mechanism to for a dynamic multi-period auto-carrier transportation problem which considers balancing vehicle usage and demand in dynamic settings. \cite{wen2010dynamic} studied dynamic multi-period vehicle routing problem with multi-objective of minimizing customer waiting time and total travel costs as well as balancing the daily workload. Historical data are used to estimate the average daily workload over the rolling horizon. 


Moreover, machine learning are also applied in wide variety of problems in transportation and logistics.
\cite{zhang_data-driven_2011} summarized a survey on data-driven intelligent traffic systems where computer vision and other learning methods for environment sense and prediction are adapted. 
\cite{zantalis_review_2019} presented a review on machine learning and IoT in smart transportation, while \cite{anuar_vehicle_2019} studied a review  on machine learning and VRP methods
in humanitarian logistics.
 
\subsubsection{Learning to Configure Algorithms}
There are a great number of hyper-parameters in VRP algorithms such as acceptance criteria of simulation annealing algorithm or population size of family of bioinspired algorithms. Usually, these hyper-parameters need to be carefully adjusted manually. Good default parameters could significantly affect the performance of algorithms \citep{bengio_machine_2020}. Finding such suitable parameters is generally called parameter setting problem (PSP). Machine learning techniques could also be used automatically to tackle the PSP problem  and are basically data-driven approaches. The general idea is to train regression models that map the specific problem instance features to the algorithm parameters where the training data are sets of pre-adjusted parameters and their performance.

\cite{calvet2016statistical} proposed a novel statistical learning-based methodology for solving the PSP and such approach was used to fine-tune the existed algorithm for multi-depot vehicle routing problem. \cite{kadaba_integration_1991} proposed a hybrid framework to solving routing and scheduling 
applications including machine learning and knowledge-based systems. In such system, 
neural networks are used for model selection and GA hyper-parameters tuning. Nevertheless, \cite{liu_machine_2017}
used simple clustering techniques to improve the parameter selection for GA. \cite{vzunic2020adaptive} built a framework where the predictive models, say support vector machine, were used to adaptively control the hyper-parameters for each instance based on the historical data. The framework’s performance was demonstrated by testing on heterogeneous fleet vehicle routing problem with time windows (HVRPTW) along with a set of realistic logistic constrains.  

Clustering technique are also used in VRP modelling. \cite{hu2007intelligent} proposed a novel framework for solving CVRPTW. In the first stage of this framework, customers are clustered into different groups based on their features. The experiments demonstrated such clustering could efficiently support the subsequent stages to generate feasible solutions. \cite{costa2020cluster} used a Cluster-based Hyper-Heuristic (CbHH) that adaptively cluster the customers to determine the neighborhood searching space at each step. The genetic algorithm is used to evolve the sequence of low-level perturbative operator to improve the initial solution. The experiment showed the effectiveness of the clustering technique and GA-based heuristic search. Similarly, \cite{gocmen_transportation_2019} used clustering method and upstream 3D-bin packing to provide context for VRP problem.



==> _robust.tex <==
 %In real case, some inputs in VRP is stochastic, such as customer demand, travel time, presence of the customer, and service time. When the demands are uncertain the problem can be modeled as the Capacitated Vehicle Routing Problem with Stochastic Demands (CVRPSD) 
 Stochastic programming assumes that the probability distribution of uncertainty is known, and aims for the best average performance over all possible future scenarios. By contrast, robust optimization assumes that the probability distribution of uncertainty can be unknown, but the range of uncertain data is known, and aims for a solution that could work even in the worst-case scenario. In general, robust optimization are considered as risk-averse methods. 
 
 %In real cases, CVRP with uncertain customer demands are often modelled as CVRP with stochastic demands, where the demand constraints may be violated when the real demands are revealed, causing a route failure in the a-priori route plan. There are different ways, called corrective actions or recourse functions, to deal with a route failure such as a detour-to-depot or a preventing restocking. It can be said that corrective actions represent extra costs to the a-priori route plan cost. That is how the concept of robustness emerged in the stochastic VRP concept. 
 %The recourse formulations model the vehicle routes as here-and-now decisions that are chosen before the uncertain customer demands are realized, whereas the recourse decisions are taken once the customer demands are observed. Most of the exact solution techniques for the stochastic CVRP with recourse rely on variants of the integer L-shaped method or branch and price algorithms (\citet{Gounaris2013}).
%The chance-constrained CVRP considers here and now vehicle routes that satisfy the customer demands along each route with a pre-specified probability. This problem is typically solved using branch-and-cut methods. 
Robust CVRPs require the vehicle routes to be feasible for all customer demands within a prespecified uncertainty set (e.g., a box, polyhedron, or ellipsoid). Branch-and-cut schemes for the exact solution of the robust CVRPs have been proposed by \citep{Ilgaz2008} and \citep{Gounaris2013}. The robust CVRPs are amenable to solution schemes that appear to scale better than those for the chance constrained CVRPs. However, the solutions obtained from the robust CVRPs can be overly conservative since all demand scenarios within the uncertainty set are treated as equally likely, and the routes are selected solely in view of the worst demand scenario from the uncertainty set(\citet{ghosal2020distributionally}). 

%Moreover, similar to stochastic programming, robust optimization models the uncertain parameters of an optimization model as random variables. The early literature robust optimization aims to determine minimum cost here-and-now decisions that remain feasible for any realization of the parameters over some prespecified support, such as budget sets, polyhedra, or intersections of ellipsoids. 
For a comprehensive review of robust optimization, we refer interested readers to \citep{Bertsimas2010}.
More recent contributions are some simulation based approaches, which transform the complex stochastic VRPs into a set of deterministic CVRPs, for which fast and extensively tested meta-heuristics exists \citep{Marcella2020}. To our knowledge, very little, if any, research has been conducted so far to apply machine learning techniques to robust VRPs, and research opportunities therefore abound in this direction.



  %In the context of the CVRPSD, there are mainly two approaches to achieve robustness: Stochastic Programming (SP) and Robust Optimization (RO), but they perceive robustness different. SP divides the set of decisions into two groups. Decisions that have to be taken before the realization of the stochastic inputs are called ﬁrst-stage decisions, whereas decisions that are made after the realization are called second-stage decisions (Birge and Louveaux 2011). In SP, feasibility constraints are relaxed and can thus be violated by perturbations on the demands. First stage decisions for which the constraints do not hold as the true value of the demands are revealed, can afterward be repaired by corrective actions (second-stage decisions). The goal of SP models is to minimize the cost of both ﬁrst-stage and second-stage decisions (Adulyasak and Jaillet 2015). For SP a solution is said to be robust when it needs less recourse cost for dealing with the true value of the stochastic input (recoverable robustness). 
  %On the other hand, RO assumes only a single period when all decisions have to be taken before the uncertain input is realized. Instead of seeking to immunize the solution in some probabilistic sense to stochastic uncertainty, RO aims at strict robustness, i.e. RO cares about designing a solution that is feasible for any realization of the uncertainty in a given set (Bertsimas, Brown, and Caramanis 2010). The works of Sungur,Ordóñez,andDessouky(2008) (Lee,Lee,and Park 2012), Gounaris, Wiesemann, and Floudas (2013b), Sun and Wang (2015), and Gounaris et al. (Gounaris et al. 2013a) deal with uncertainties in the demands in the SCVRP via RO. Apart from assuming that the probability distributions modeling the demands are available, SP suﬀers from other drawback: it is aﬀected by the.


==> _stochastic.tex <==

Machine learning has long been used to assist the modelling of stochastic VRPs, where the uncertain data is represented by random variables with known probability distributions. A number of studies have modelled stochastic VRPs as a Markov
 Decision Process (MDP), which is closely connected to Neuro-Dynamic Programming (NDP). NDP is also referred to as reinforcement learning in the artificial intelligence literature \citep{bertsekas_neuro-dynamic_1996}. The value-function approximation method and/or the policy-function approximation method of NDP is tailored in each of those studies. \cite{secomandi_comparing_2000} compares two different NDP algorithms on solving VRPs with stochastic demands and shows that the NDP with rollout policy performs better than an approximate policy iteration.
\cite{godfrey_adaptive_2002} formulate the dynamic fleet management 
problem as a multistage dynamic program and use gradient-based information to obtain nonlinear approximations of value functions.
\cite{zhang2013single} uses tabular value approximation 
and policy approximation to solve VRPs with stochastic demands.
\cite{ulmer2020modeling} present a literature review of and modeling framework for dynamic VRP  and proposed a new
route-based MDP model that extends the conventional MDP model for dynamic and stochastic optimisation problems by redefining the conventional action space to operate on route plans.


Machine learning has also been used to estimate the probability distributions of uncertain data in stochastic VRPs. 
\cite{talbi_hybrid_2013} state that hybrid metaheuristics are often used to solve complex and
large real-world optimization problems, combining advantages from machine learning techniques and mathematical optimisation. The authors examine the hybrid metaheuristics for dynamic stochastic VRP, where not all information is available in advance.
%ensembled machine learning and other metaheuristics to discuss hybrid metaheuristics for dynamic and stochastic vehicle routing. Some recent research interest by the time the book is published and application in complex real-world problems.
%Moreover, evolution algorithm based method by \cite{van_hemert_dynamic_2004} is applied to solve dynamic routing problem, for it could adapt to the environment change. 
\cite{bent2005online} proposed to use machine learning approach by sampling 
from historical data to get partial knowledge of stochastic distribution in online 
scheduling problems. They claim such approach could help widen the application area of stochastic algorithms. Experiment are made on several problems including dynamic VRPTW from previous work \cite{bent_scenario-based_2004}.
\cite{defourny_machine_2010}  generated and selected scenario trees with random
branching structures for multistage Stochastic Programming over large planning horizons. This work combine the perturb-and-combine estimation methods from machine learning with stochastic programming techniques for sequential decision making under uncertainty. The performance has been shown quite good.

==> iterative.tex <==
\section{Iterative}



==> localSearch.tex <==
%this file is not used any more. The contents have been merged into Section 3.2

Machine-learning model could be used to perturb solution. For example, take a complete solution as input and indices of node could be modified as output. In this case, machine learning model (usually neural network) itself acts as perturbative heuristic in the traditional optimization algorithm. 

\cite{da2020learning} focused on improvement (or perturbative) heuristics that could refine a given solution iteratively until reaching a near-optimal solution. In his work, a method that could learn a policy to generate the 2-opt heuristic for TSP was proposed. A similar encoder-decoder framework was used to encode the graph and generate a sequence of action distribution but the mechanism was modified to make it easy to extend to k-opt operations. The difference to the initial pointer network is that at each decoder step, the model output an action (two nodes for 2-opt) rather than one specific node to construct the final solution. 
 
\cite{gao2020learn} proposed a method for learning the local search heuristics. Similarly, an encoder-decoder was used and trained by actor-critic algorithm. Inspired by the large neighborhood search (LNS) algorithm for vehicle routing problems \citep{shaw1998using}, the authors defined the local search heuristic as a destroy operator and a repair operator. The destroy operator removed a subset node of the current solution and the repair operator was used to generate a permutation of the selected elements and insert them back. Motivated by the graph attention network (GAT) mechanism \citep{velivckovic2017graph} which is an effective method to represent the graph topology by propagating the neighbor node information through the attention mechanism, the authors proposed a modified version called Element-wise GAT with Edge-embedding (EGATE) which not only considered the information of nodes but also the arc between the nodes. The attention mask was generated by softmax the concatenation of embedding of arc and two nodes it connected with. The decoder acted as destroy and repair operation.

\cite{chen2020dynamic} were also motivated by LNS algorithm, and proposed a similar method called dynamic particle removal (DPR) using Hierarchical Recurrent Graph Convolutional Network (HRGCN). Similar to the method of \cite{gao2020learn}, the authors also defined the local search as a destroy and repair operator. The degree (size and the allocation of the sub-nodes) of the destroy operator was dynamically determined. The HRGCN is able to be aware of spatial (graph topology) and temporal (embedding in previous iterations) context information. 

Another learning-based LNS algorithm proposed by \cite{hottung2019neural} was called neural large neighborhood search (NLNS). The method was specifically adapted to support parallel computing, which is one of the contributions of this method. Such features could support two implement patterns: batch search which solved a set of instances simultaneously and the single instance search which solved only one instance concurrently. The method was demonstrated by capacitated vehicle routing problem (CVRP) and the split delivery vehicle routing problem (SDVRP).

\cite{chen2019learning} proposed a general method for combinatorial optimisation problems called local rewriting framework (Neuwriter) which generates a solution iteratively. In this work, a region picker and a rule picker were defined and trained separately. At each rewrite step, two pickers selected a sub-area of current solution and its rewrite rule one behind the other. Then the modified sub-area will be put back to generate a new solution. The model repeated this process until convergence. The online job scheduling problem, expression simplification problem, and capacitated vehicle routing problem were used to test this method. A bi-directional LSTM layer was used to embed the input nodes in CVRP problem, and a similar pointer network mechanism was used to select a node through a probability distribution. 

Neuwriter \citep{chen2019learning} is effective for iteratively refining a given solution and performs better than the constructive methods. However, in Neuwriter framework, two policies (region select policy and rule select policy) need to be learned which make the training process a little bit cumbersome. To tackle this problem, \cite{wu2019learning} integrated two policy networks into one. Specifically, the compatibility computation was adopted in the model to produce a probability matrix of node pairs whose element specified the two corresponding nodes. In order to capture the node position information, sinusoidal positional encoding was introduced to the embedding layer. Moreover, the mechanisms of batch normalization and skip connection \citep{he2016deep} were adopted in the model. The results showed that this method outperformed Neuwriter. 

        \subsubsection{Learning to Select Heuristics}

Machine-learning model could also perturb solution indirectly by selecting from a set of predefined heuristics. Such a mechanism is called `Heuristic Selection' in hyper-heuristic family based on the classification of \cite{burke2019classification}. Another corresponding mechanism called `Heuristic Generation' will be introduced in next subsection. Heuristic selection could be based on meta-heuristic, reinforcement learning, choice function or random selection.

Heuristic-selection policy could also be learned from existing examples. \cite{tyasnurita2017learning} used a time delay neural network (TDNN) as a classifier to select the low-level heuristics to solve open vehicle routing problem. Parameters of TNDD were optimized by imitating the behaviors of an ‘expert’ hyper-heuristic algorithm called MCF-AM (Modified Choice Function - All Moves) \citep{drake2012improved} running on the training problem instances. The trained network was used to solve unseen instances.

In order to balance the distance of each route, \cite{hidayatul2019solving} conduced hyper-heuristic method to solve multi-objective optimization of vehicle routing problem with time windows. In this research, hill climbing, and great deluge were used as move acceptances for accepting selected heuristic. Low level heuristics were selected randomly. Number of non-dominated Pareto fronts and coverage are two indicators to judge the performance in the experiments.

\cite{sabar2014dynamic} proposed a hyper-heuristic method called Gene Expression Programming based Hyper-Heuristic (GEP-HH) framework and used it to solve the dynamic vehicle routing problem. In this method, the low-level heuristics were selected by a mechanism called dynamic multiarmed bandit (DMAB) extreme-value-based reward \citep{fialho2010analyzing}. The acceptance criterion for each problem instance was automatically generated by a gene expression programming framework.

Another similar method also proposed by \cite{sabar2014automatic} used gene expression programming to generate high-level heuristic based on the information of the problem states. The method was tested on six different combinatorial optimization problems included VRP with HyFlex \citep{ochoa2012hyflex}  which is a well-known hyper-heuristic algorithm framework. 


Reinforcement learning is a suitable technique to train low-level heuristic-selection policy. \cite{lu2019learning} proposed an iterative improvement method called `Learn to Improve (L2I)' based on that. Notably, this method outperformed LKH3 \citep{helsgaun2017extension} which was the state-of-the-art method of VRP on both speed and solution quality. The model started with a random initial solution and used two classes of predefined low-level heuristics, namely, improvement operators and perturbation operators which were used to local search the solution and destroy part of the solution respectively. A double layer controller guided by reinforcement learning was used to select the corresponding heuristics. When generating the action, the model would also consider the history actions and their effects. A policy ensemble mechanism was used to improve the generalization.
 
        \subsubsection{Learning to Generate Heuristics}
        
In hyper-heuristic framework, the low-level heuristics could also be generated during the execution of the model rather than predefined. Most of the approaches are evolving genetic decision trees built from low-level heuristics.   
        
\cite{jacobsen2017evolving} attempted hyper-heuristic method to solve Dynamic Vehicle Routing with Time Windows (DVRPTW). Such problems require the accepting or rejecting decisions for dynamically arrived customer requests. The genetic programming evolved heuristics were used to accept new requests and add them to the current routes. The result showed that with the dynamism degree increasing, the GP-evolved heuristics significantly outperformed the handcrafted heuristics.

To gain more interpretable routing policies, \cite{wang2019evolving} used three ensemble genetic programming method, namely, Bagging GP, Boosting GP, and Cooperative Co-evolution GP to solve uncertain capacitated arc routing problem. Evolved depth-limited tree expressions are ensemble with these methods to represent the priorities of each task in an instance. The results showed that ensemble of simple policies is able to compete the complex policies while maintain their high interpretability. 

